StaticFixer: From Static Analysis to Static Repair

Static analysis tools are traditionally used to detect and flag programs that violate properties. We show that static analysis tools can also be used to perturb programs that satisfy a property to construct variants that violate the property. Using this insight we can construct paired data sets of unsafe-safe program pairs, and learn strategies to automatically repair property violations. We present a system called \sysname, which automatically repairs information flow vulnerabilities using this approach. Since information flow properties are non-local (both to check and repair), \sysname also introduces a novel domain specific language (DSL) and strategy learning algorithms for synthesizing non-local repairs. We use \sysname to synthesize strategies for repairing two types of information flow vulnerabilities, unvalidated dynamic calls and cross-site scripting, and show that \sysname successfully repairs several hundred vulnerabilities from open source {\sc JavaScript} repositories, outperforming neural baselines built using {\sc CodeT5} and {\sc Codex}. Our datasets can be downloaded from \url{http://aka.ms/StaticFixer}.

==> algomacros.tex <==
%%%%%%%%% my function definitions formatting
\algblockdefx[myFuncBlock]{myFuncStart}{myFuncEnd}%
[2]{\underline{\textsc{#1}} (#2)}%
[0]{}

\makeatletter
\ifthenelse{\equal{\ALG@noend}{t}}%
  {\algtext*{myFuncEnd}}
  {}%
\makeatother


\newcommand{\myFunctwo}[2]{\myFuncStart{#1}{#2}\myFuncEnd} 
\newcommand{\myFunc}[2]{\Statex \underline{\textsc{#1}} (#2)} 

%%%%%%%%%% 
\newcommand{\emptylist}{empty \textbf{list}}
\newcommand{\emptydict}{empty \textbf{dict}}
\newcommand{\algout}[1]{\textbf{out} #1}

%%%%%%%%%% my (attempt) at for loop
\algloopdefx{myFor}[2]{\textbf{for each} $#1 \in #2$:}

\algcblockdefx[myForBlock]{myFor}{Eeee}{myForEnd}
[1]{\textbf{Eeee} "#1"}
{}


%%%%%%%%%
\renewcommand\algorithmicthen{:}
\renewcommand\algorithmicdo{:}

\makeatletter
\newcommand\fs@ruled@notop{\def\@fs@cfont{\bfseries}\let\@fs@capt\floatc@ruled
  %\def\@fs@pre{\hrule height.8pt depth0pt \kern2pt}% <----removed
  \def\@fs@pre{}%
  \def\@fs@post{}%
  \def\@fs@mid{}%
  %\def\@fs@post{\kern2pt\hrule\relax}%
  %\def\@fs@mid{\kern2pt\hrule\kern2pt}%
  \let\@fs@iftopcapt\iftrue}
\renewcommand\fst@algorithm{\fs@ruled@notop}
\makeatother




==> architecture.tex <==
\begin{figure*}[!t]
\begin{tikzpicture}[every node/.style={inner sep=3}]
\node[draw, rectangle, ultra thick] (n1) { \begin{tabular}{c} Static Analysis \\ Witnessing \end{tabular} } ;
\node[draw, rectangle, ultra thick, right of=n1, xshift=2.5cm] (n2) {\begin{tabular}{c} Witness \\ Removal \end{tabular}} ;
\node[draw, rectangle, ultra thick, right of=n2, xshift=2cm] (n3) {\begin{tabular}{c} Strategy \\ Learning \end{tabular}} ;
\node[draw, rectangle, ultra thick, right of=n3, xshift=2cm] (n4) {\begin{tabular}{c} Strategy \\ Application \end{tabular}} ;

%\path[draw,->] (n1) -- (n2) ;
%\path[draw,->] (n2) -- (n4) ;
\end{tikzpicture}
\caption{Overview of \sysname ; Right now incorrect - partly because we don't have a proper/formal ranking module}
\label{fig:staticfixer-architecture}
\vspace{-0.3cm}
\end{figure*}

==> astsyntax.tex <==
\setlength{\grammarindent}{5em} % increase separation between LHS/RHS

\begin{figure}
\begin{align*}
        \DRulenew{}{Set of Nodes}{\ensuremath{\mathcal{N}}}\ \text{::=}&\ \{n_0,\ldots,n_k\} \\
        \DRulenew{}{Node}{\I{n}}\ \text{::=}&\ \mathit{id}\in\mathbb{N} \\
        \DRulenew{}{Integer}{\I{z}}\ \text{::=}&\ -1,0,1,\ldots \\
        \DRulenew{}{\astree edge type}{\edgetype\ensuremath{'}}\ \text{::=}&\ \T{SynParent}\ \ |\ \ \T{SynChild} \\
        \DRulenew{}{\astree edge}{e\ensuremath{'}}\ \text{::=}&\ (n_1,n_2,\edgetype',z) \\
        \DRulenew{}{Set of \astree edges}{\ensuremath{\mathcal{E}'}}\ \text{::=}&\ \{e_0',\ldots,e_k'\} \\
        \DRulenew{}{\pdg edge type}{\edgetype}\ \text{::=}&\ \edgetype'\ \ |\ \ \T{SemParent}\ \ |\ \ \T{SemChild} \\
        \DRulenew{}{\pdg edge}{e}\ \text{::=}&\ (n_1,n_2,\edgetype,z) \\
        \DRulenew{}{Set of \pdg edges}{\ensuremath{\mathcal{E}}}\ \text{::=}&\ \{e_0,\ldots,e_k\} \\
        \DRulenew{}{Annotations of \pdg}{A}\ \text{::=}&\ (n,\T{source}) \ \ |\ \ (n,\T{sink})\ \ |\ \ (n,\T{sanitizer})\ \ |\ \ (n,\T{guard}) 
        \end{align*}
    \caption{Nodes and edges of \astree  and \pdg. The primes are usually omitted  for brevity.}
    \label{fig:astsyntax}        
\end{figure}




==> dataterms.tex <==
\begin{figure}[!h]
\small
\begin{alltt}
\textit{ast} :- \textsc{Node}(\textit{type}, \textit{value}, \textit{ast1}, \textit{ast2}, ...)
\textit{type} :- string
\textit{value} :- string
\textit{annotast} :- \textsc{AnnotNode}(\textit{ast}, \textit{semedges})
\textit{semedges} :- \textit{semedge} | \textit{semedges} ; \textit{semedge}
\textit{semedge} :- SemanticEdge(\textit{annotast}, \textit{annotast})

\end{alltt}
\vspace{-2ex}
\caption{Definitions for \astree and \pdg}
\label{fig:data-terminology}
\end{figure}


==> ql.tex <==
\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.48\textwidth}
    \begin{lstlisting}[escapechar=@,autogobble]
    class ReflectedXSSConfig{
      Configuration() { this = "ReflectedXSSConfig"; }
      isSource(Node src) => {
        src instanceof ServerInput 
      }
      isSink(Node sink) => {
        sink instanceof HttpResponse
      }
      isSanitizer(Node san) => {
        san instanceof EscapeSanitizer
      }
      isGuard(Node guard) => {
        san instanceof QuoteGuard or
        san instanceof ContainsHtmlGuard
      }
    }
    
    from ReflectedXSSConfig cfg, Node src, Node sink
    where cfg.hasFlow(src, sink)
    select src, sink
    \end{lstlisting}
    \caption{\sa configuration for \xss}\label{fig:configuration}
    \end{subfigure}\hfil%
    \begin{subfigure}{0.48\textwidth}
    \begin{lstlisting}[escapechar=@,autogobble]
    class SafeConfig extends ReflectedXSSConfig {
      SafeConfig() { this = "SafeConfig" }
      isSource(Node src) => super.isSource(src)
      isSink(Node sink) => super.isSink(sink)
      isSanitizer(Node san) => none()
      isGuard(Node guard) => none() 
      isWitness(Node src, Node sink, Node witness, string type){
        (super.isSanitizer(witness) and type="san" or
        super.isGuard(witness) and type="guard") 
        and 
        src.succ() = witness and 
        witness.succ() = sink
      }
    }
    
    from SafeConfig cfg, Node src, Node sink, 
         Node witness, string type
    where cfg.hasFlow(src, sink) and 
          cfg.isWitness(src, sink, witness, type)
    select src, sink, witness, type
    \end{lstlisting}
    \caption{\sa-witnessing configuration for \xss }\label{fig:safe-configuration}
    \end{subfigure}
    \caption{Simplified configurations detecting unsafe and safe code for \xss respectively. Note that to do this using \codeql, we need to take additional measures to block the taint flows appropriately. We share the actual \codeql queries in the Appendix~\ref{app:codeql-queries}}
    \label{fig:configuration-vs-safe-configuration}
\end{figure}


==> synthesisalgo.tex <==
%O := \{\(\strategy\sb{1},\strategy\sb{2},\dots,\strategy\sb{k}\)\}
\HUGE DONT USE THIS - USE synthesisalgo2
\begin{figure*}

\begin{subfigure}{0.49\textwidth}
\normalsize
\begin{alltt}
{\footnotesize{\internallinenumbers \underline{\textsc{Learn}}(\(I \equiv \{(\prog\sb{1},\concedit\sb{1}),(\prog\sb{2},\concedit\sb{2}),\dots,(\prog\sb{n},\concedit\sb{n})\}\)
for each \((\prog\sb{i},\concedit\sb{i}) \in I\):
    \textsc{PreprocessConcEdit}(\(\prog\sb{i},\concedit\sb{i}\))
\(pairIndices \leftarrow\) \textsc{PairSimilar}(I)
for each \(i, j \in pairIndices\):
    \textbf{output} \textsc{MergeEdits}(\(\concedit\sb{i},\concedit\sb{j}\))

\underline{\textsc{PreprocessConcEdit}}(\(\prog,\concedit\))
\(editpaths \leftarrow\)  \textsc{GetEditLocPaths}(\(\prog,\concedit\))
\(\concedit.paths \leftarrow editpaths\)
\(\concinsertcode \leftarrow \concedit.editcode\)
for each \(node \in \concinsertcode\):
    \(node.refs \leftarrow empty \textbf{dict}\)
    for each \(\conceditpath \in editpaths\):
        \(refpaths \leftarrow\) \textsc{GetRefPaths}(\(\prog,\conceditpath, node\))
        \(node.refs[\conceditpath] \leftarrow refpaths\)

\underline{\textsc{GetEditLocPaths}}(\(\prog,\concedit\))
\(\conceditloc \leftarrow \concedit.editloc\)
\(source \leftarrow \prog.source\)
\(paths \leftarrow\) \textsc{BiDirecBFS(\(source, \conceditloc\))}
for each \(\conceditpath \in paths\):
    \(\conceditpath.semLoc \leftarrow\) \textsc{GetSemanticLoc}(\(\conceditpath\))
\textbf{output} paths

\underline{\textsc{GetSemanticLoc}}(\(\conceditpath\))
for each \(edge\) in \(\conceditpath\):
    if \(edge.type\) = ast:
        \textbf{output} \(edge.endnode\)
\textbf{output} \(\conceditpath.endnode\)

\underline{\textsc{GetRefPaths}}(\(\prog,\conceditpath, node\))
\(semLoc \leftarrow \conceditpath.semLoc\)
\(val \leftarrow node.val\)
\(refpaths \leftarrow\) \textsc{MaxLevelBFS}(\(\prog, semLoc, val\))
\textbf{output} refpaths

\underline{\textsc{PairSimilar}}(\(I \equiv \{(\prog\sb{1},\concedit\sb{1}),(\prog\sb{2},\concedit\sb{2}),\dots,(\prog\sb{n},\concedit\sb{n})\}\))
\(scoreList \leftarrow\) empty \textbf{list}
for each \(i \in 1 \dots n\):
    for each \(j \in 1 \dots n\):
        \(\concinsertcode\sb{i},\concinsertcode\sb{j} \leftarrow \concedit\sb{i}.editcode, \concedit\sb{j}.editcode\)
        if \(\concinsertcode\sb{i}=\concinsertcode\sb{j}\): \(score \leftarrow 0\)
        else: \(score \leftarrow\) \textsc{ASTSimilarity}(\(\concinsertcode\sb{i},\concinsertcode\sb{j}\))
        scoreList.append((score,i,j))
\(scoreList \leftarrow\) \textsc{Sort}(\(scoreList\))
\textbf{output} scoreList.indices
}}
\end{alltt}
\end{subfigure}\hfil%
\begin{subfigure}{0.49\textwidth}
\normalsize
\begin{alltt}
{\footnotesize{\internallinenumbers \underline{\textsc{MergeEdit}}(\(\concedit\sb{i}, \concedit\sb{j}\))
\(mergedPaths \leftarrow\) \textsc{MergePaths}(\(\concedit\sb{i}.paths, \concedit\sb{j}.paths\))
for each \(\editpath \in mergedPaths\):
    \(semLocs \leftarrow \editpath.semLocs\)
    

}}
\end{alltt}
\end{subfigure}
\caption{Sketch of our strategy learning algorithm}
\label{fig:strategy_learning}
\end{figure*}
